The effect of a solar flare on chromospheric oscillations

Oscillations in the solar atmosphere have long been observed in quiet conditions, and increasingly also in data taken during solar flares. The chromosphere is known for its 3-minute signals, which are particularly strong over sunspot umbrae. These signals are thought to be driven by photospheric disturbances and their periods determined by the chromosphere's acoustic cut-off frequency. A small number of observations have shown the chromospheric 3-minute signals to be affected by energetic events such as solar flares, however the link between flare activity and these oscillatory signals remains unclear. In this work we present evidence of changes to the oscillatory structure of the chromosphere over a sunspot which occurs during the impulsive phase of an M1 flare. Using imaging data from the CRISP instrument across the H$\alpha$ and Ca II 8542 {\AA} spectral lines, we employed a method of fitting models to power spectra to produce maps of areas where there is evidence of oscillatory signals above a red noise background. Comparing results taken before and after the impulsive phase of the flare, we found that the oscillatory signals taken after the start of the flare differ in two ways: the locations of oscillatory signals had changed and the typical periods of the oscillations had tended to increase (in some cases increasing from $\lt$100s to $\sim$200s). Both of these results can be explained by a restructuring of the magnetic field in the chromosphere during the flare activity, which is backed up by images of coronal loops showing clear changes to magnetic connectivity. These results represent one of the many ways that active regions can be affected by solar flare events.

==> old_files/data.tex <==
\section{Data processing}
The CRISP data is in FITS format and is in dimensions ($\lambda$, x, y) with (x, 
y) = (1398, 1473), 0.057" per pixel. For H-alpha the $\lambda$ dimension covers $\pm 1.4\rm{\AA}$ in steps of $0.2\rm{\AA}$ and ca8542 covers $\pm 1.2\rm{\AA}$ in steps of $0.1\rm{\AA}$.

Two $\sim$30 minute periods before and after the flare peak are analysed. The pre- and post-flare periods cover frames 253 to 400 and 470 to 617 respectively, or 16:16 to 16:45 and 16:58 to 17:27, with an average cadence of 11.6 seconds.

\subsection{Masking}
The CRISP field of view rotates and moves, to track features in the images. This means that features stay in the same group of pixels throughout the observation but some pixels do not always contain image data. For this reason pixels are selected for analysis which contain data over the entire pre- or post-flare windows. This was achieved by first creating a mask from each individual frame by selecting which pixels contained data (assigned value 1) and which were outside the field of view (assigned 0). Every frame was then multiplied together, to obtain two master masks for each $\sim$30 minute pre- and post-flare period.

\subsection{Re-binning}
The analysis will be performed on individual timeseries from each pixel in the masked field of view, so to reduce computing time and smooth out noise, the images were re-binned by a factor of 10. The x- and y-dimensions were first reduced to a multiple of 10 by clipping the edges off (8 pixels on the x-dimension and 3 on the y-dimension) and then summing over 10 by 10 grids of pixels creating 139 by 147 images. This process was also applied to the masks which were obtained previously.

\subsection{Cubing}
Single wavelength points were isolated, then re-binned and combined into cubes with dimensions (t, x, y).


\subsection{Examples of fits}
for 1600, use row/col = 80/23, also row 90, column 45 Halpha core pre flare

\begin{figure}[hbtp]
    \centering
    \includegraphics[width=1\linewidth]{bad_fit_single_pix.pdf}
    \caption{A bad fit obtained from a single pixel in the penumbra of the main sunspot}
    \label{fig:badfit}
\end{figure}

\begin{figure}[hbtp]
    \centering
    \includegraphics[width=1\linewidth]{3x3_avg_fit.pdf}
    \caption{PSD averaged over a 3x3 box centred on the same pixel as figure \ref{fig:badfit}}
    \label{fig:my_label}
\end{figure}
